Making Quantum Local Verifiers Simulable with Potential Applications to Zero-Knowledge

Recently Chen and Movassagh proposed the quantum Merkle tree, which is a quantum analogue of the well-known classical Merkle tree. It gives a succinct verification protocol for quantum state commitment. Although they only proved security against semi-honest provers, they conjectured its general security. Using the proposed quantum Merkle tree, they gave a quantum analogue of Kilian's succinct argument for NP, which is based on probabilistically checkable proofs (PCPs). A nice feature of Kilian's argument is that it can be extended to a zero-knowledge succinct argument for NP, if the underlying PCP is zero-knowledge. Hence, a natural question is whether one can also make the quantum succinct argument by Chen and Movassagh zero-knowledge as well. This work makes progress on this problem. We generalize the recent result of Broadbent and Grilo to show that any local quantum verifier can be made simulable with a minor reduction in completeness and soundness. Roughly speaking, a local quantum verifier is simulable if in the yes case, the local views of the verifier can be computed without knowing the actual quantum proof; it can be seen as the quantum analogue of the classical zero-knowledge PCPs. Hence we conjecture that applying the proposed succinct quantum argument of Chen and Movassagh to a simulable local verifier is indeed zero-knowledge.

==> backup.tex <==

In this section we give a high-level overview for our first result: a zero-knowledge proof protocol for $(k,\eps)$-$\projLH$.

	\paragraph*{Notation.} We will use $\data$ to denote the $n$-qubit register storing a potential witness to $(k,\eps)$-$\projLH$, and $\out$ be a single-qubit output register. Given a state $\spz{\phi} \in \Hdata$, we use $V_{\Pi_i}$ to denote the following unitary acting on $\Hdata \otimes \Hout$:
	\[
	V_{\Pi_i} ( \spz{\phi}_\data \spz{b}_\out) = \Pi_i \spz{\phi}_\data \spz{b}_\out + (I - \Pi_i)\spz{\phi}_\data \spz{b \oplus 1}_\out.
	\]
	
	Clearly, for $\spz{\phi} \in \Hdata$ such that $\Tr[\Pi_i \phi] = 0$, we have
	\[
	V_{\Pi_i} ( \spz{\phi}_\data \spz{0}_\out) = \spz{\phi}_\data \spz{1}_\out.
	\]

	We aim to first prove the following warm-up theorem.

	\begin{theorem}\label{theo:warm-up}
		For any $k \in \N$ and constant $\eps \in (0,1)$, there is a constant round zero-knowledge proof protocol for $(k,\eps)$-$\projLH$ with completeness $1$ and soundness $1-\Omega(1)$.
	\end{theorem}
	\cljnote{Eventually need to get soundness $1/n^c$ for every $c$ by repetition, and also deal with $\LH$ instead of $\projLH$. Both steps are straightforward but tedious, I am going to ignore this issue for now.}
	
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,
		semithick,scale = 2.0]
		\tikzstyle{every state}=[text=black,rectangle, text width=4.5cm]
		\tikzstyle{arrow}=[thick]
		
		\node [state] (VanV) at (0, 0) {\footnotesize Vanilla verifier $\Vvanilla$ for $(k,\eps)$-$\projLH$ };
		
		\node [state] (VanHV) at (5,0) {\footnotesize Vanilla history verifier $\VHvanilla$ for $(k,\delta)$-$\History$-$\projLH$};
		
		\node [state] (EncV) at (0,-2) {\footnotesize Encoded verifier $\Venc$ for $(k,\eps)$-$\EncprojLH$};
		
		\node [state] (EncHV) at (5,-2) {\footnotesize Encoded history verifier $\VHenc$ for $(k,\delta)$-$\History$-$\EncprojLH$};
		
		\draw[arrow] (VanV)  edge node {\footnotesize Circuit-to-Hamiltonian for $\Vvanilla$}  (VanHV);
		\draw[arrow] (EncV)  edge node {\footnotesize Circuit-to-Hamiltonian for $\Venc$}  (EncHV);
		\draw[arrow] (VanV)  edge node {\footnotesize Fault-Tolerance version of $\Venc$}  (EncV);
		
		%\draw[arrow] (avghardPSPACE) -- (aaeAvgMA);
		%\draw[arrow] (PSPACEcomplete) -- (aaeAvgMA);
		%\draw[arrow] (aaeAvgMA) -- (weakavglowerbound);
		%\draw[arrow] (weakavglowerbound) edge node {mild to strong hardness amplification} (strongavglowerbound);
		\end{tikzpicture}
		
		\caption{The structure of the reduction}
		\label{fig:structure}
	\end{figure}

To prove~\autoref{theo:warm-up}, our goal is to construct a reduction from $(k,\eps)$-$\projLH$ to another problem $(k,\delta)$-$\History$-$\EncprojLH \in (2,O(\log m))\text{-}\SimQMA$ with completeness $1$ and constant soundness. A simple zero-knowledge protocol can be constructed for $(k,\delta)$-$\History$-$\EncprojLH$ by adapting techniques in~\cite{BroadbentG20}.
	
	In~\autoref{sec:van-verifier}, we describe the vanilla verifier $\Vvanilla$ and its corresponding history verifier $\Vvanilla$. This steps servers as a toy example of the later transformation.
	
	In~\autoref{sec:enc-verifier}, we describe the encoded verifier $\Venc$ which is the fault-tolerance version of the $\Vvanilla$, together with its corresponding history verifier $\VHenc$. $\VHenc$ would be the simulatable verifier of our target language $(k,\delta)$-$\History$-$\EncprojLH \in (2,O(\log m))\text{-}\SimQMA$. Formally, we prove the following theorem in~\autoref{sec:enc-verifier}.
	
	\begin{theorem}\label{theo:history-problem-prop}
		For every $\eps > 0$, there is a constant $\delta > 0$ such that the followings hold for the $(k,\delta)$-$\History$-$\EncprojLH$ problem.
		\begin{itemize}
			\item (\textbf{Reduction from $(k,\eps)$-$\projLH$}) There is a reduction $\redEncH$ from $(k,\eps)$-$\projLH$ to $(k,\delta)$-$\History$-$\EncprojLH$, such that for a $(k,\eps)$-$\projLH$ instance $G$:
			\begin{itemize}
				\item $G \in (k,\eps)$-$\projLH_{\yes}$ implies $\redEncH(G) \in (k,\delta)$-$\History$-$\EncprojLH_{\yes}$.
				\item $G \in (k,\eps)$-$\projLH_{\no}$ implies $\redEncH(G) \in (k,\delta)$-$\History$-$\EncprojLH_{\no}$.
			\end{itemize}
			\item (\textbf{Simulation}) $(k,\delta)$-$\History$-$\EncprojLH$ is in $(2,O(\log m))$-$\SimQMA$ with completeness $1$ and soundness $1 - \Omega(\delta)$.
		\end{itemize}
	\end{theorem}
	
	In~\autoref{sec:general-transform}, we construct a simple commit-and-open zero-knowledge protocol for all problems in $(O(1),O(\log m))\text{-}\SimQMA$. Formally, we prove the following theorem in~\autoref{sec:general-transform}.
	
	\begin{theorem}\label{theo:general-transform}
		Let $L = (L_{\yes},L_{\no}) \in (\ell,k)\text{-}\SimQMA$ with completeness $c$ and soundness $s$. Assuming $\ell = O(1)$ and $k = O(\log n)$, there is $\ell + O(1)$-round computational zero-knowledge proof for $L$ with completeness $c$ and soundness $s$.
	\end{theorem}

	\autoref{theo:warm-up} follows as a simple corollary of~\autoref{theo:history-problem-prop} and~\autoref{theo:general-transform}.
	
	\section{The vanilla verifier and vanilla history verifier}\label{sec:van-verifier}
	
	In this section we analyze a simple vanilla verifier for $(k,\eps)$-$\projLH$, together with its corresponding history verifier $\VHvanilla$. While $\VHvanilla$ is not directly used in our final construction, we hope this section serves as warm up for the much more involved construction in~\autoref{sec:enc-verifier}.
	
	\begin{construction}{The vanilla verifier $\Vvanilla$ for $(k,\eps)$-$\projLH$}
		\begin{enumerate}
			\item (\textbf{Setup}) $\Vvanilla$ expects an $n$-qubit witness in register $\data$, and uses $2\log m + 1$ ancilla qubits consisting of $\log m$ qubits in each of registers $\idx$ and $\midx$, and $1$ qubit in register $\out$.
			
			\item $\Vvanilla$ first apply a Hadamard gate to each qubits in $\idx$.
			
			\item $\Vvanilla$ next ``measures'' $\idx$ in the following way: for each $i \in [\log m]$, it applies $\CNOT$ with control bit $\idx(i)$ and target bit $\midx(i)$.
			
			\item Then, $\Vvanilla$ applies the following unitary $U_{\sf test}$ on $\Hdata \otimes \Hout \otimes \Hidx$ as follows:
			\[
			U_{\sf test} \spz{\phi}_{\data}\spz{b}_{\out}\spz{i}_{\idx} = (V_{\Pi_i} \spz{\phi}_{\data}\spz{b}_{\out})\spz{i}_{\idx}.
			\]
			That is,
			\[
			U_{\sf test} = \sum_{i \in [m]} V_{\Pi_i} \otimes \proj{i}_{\idx}.
			\]
			\item Finally, $\Vvanilla$ measures the qubit in register $\out$ and accepts if the outcome is $1$.
		\end{enumerate}
	\end{construction}
	
	The following lemma can be shown by a straightforward calculation.
	
	\begin{lemma}
		$\Vvanilla$ rejects a given $n$-qubit witness $\sigma$ with probability exactly	$\Tr[G \sigma]$.
	\end{lemma}
	
	\subsection{The history verifier $\VHvanilla$}\label{sec:van-H-verifier}

In the following we describe a transformation from $\Vvanilla$ to another verifier $\VHvanilla$ for the history Hamiltonian obtained from $\Vvanilla$. This serves as an illustration of our later transformation.

	Note that $\Vvanilla$ can be written as a product of $T = 3$ unitaries,
	\[
	\Vvanilla = \Vvanilla_{T} \cdots \Vvanilla_1,
	\]
	where
	\[
	\Vvanilla_1 = \prod_{i \in [\log m]} H_{\idx(i)},\quad \Vvanilla_2 = \prod_{i \in [\log m]} (\CNOT)_{\idx(i),\midx(i)},\quad\Vvanilla_3 = U_{\sf test}.
	\]
	
	Let $\Hamhis$ be the history Hamiltonian of $\Vvanilla$ with $B=3$, $S_1 = \{ \idx(i) \}_{i \in [\log m]}$, $S_2 = \{ \midx(i) \}_{i \in [\log m]}$ and $S_3 = \{\out(1)\}$ ($S_1,S_2,S_3$ corresponds to qubits in $\idx$, $\midx$ and $\out$, respectively) from~\autoref{defi:history-Hamiltonians}. We finally define
	\[
	\Hamout = \proj{0}_{\out} \otimes \proj{1}_{\clock(T)},
	\]
	and set
	\[
	H = \Hamout + \Hamhis.
	\]
	
	Now we consider the following problem.
	
	\begin{construction}{$(k,\delta)$-$\History$-$\projLH$}
		\begin{itemize}
 		\item (\textbf{Input}) Given a history Hamiltonian $H$ with the guarantee that $H$ is constructed from the vanilla verifier for a certain $k$-local Hamiltonian $G = \sum_{i \in [m]} G_i$. Determine between the following two cases:
 		\begin{itemize}
 			\item (\textbf{Yes}) $\lmin(H) = 0$ or 
 			\item (\textbf{No}) $\lmin(H) \ge \delta m$.
 		\end{itemize}
 	\end{itemize}
	\end{construction}
	
	\subsubsection{Soundness analysis}\label{sec:van-soundness}
	
	\begin{lemma}\label{lemma:van-soundness}
		There exists a universal constant $c > 1$ such that, if there is a state $\spz{\Phi} \in \Hclock \otimes \Hstate$ such that $\rpz{\Phi} H \spz{\Phi} \le \delta$, then $\lmin(G) \le c \cdot \sqrt{\delta} \cdot m$.
	\end{lemma}
	\begin{proof}
	
	Let $\spz{\Phi} \in \Hclock \otimes \Hstate$ and suppose $\rpz{\Phi} H \spz{\Phi} \le \delta$, it follows from~\autoref{lemma:close-to-history} that there exists a history state $\spz{\Psi}$ such that
	\[
	\| \proj{\Phi} - \proj{\Psi} \|_1 \le O(\sqrt{\delta}).
	\]
	
	This also implies that
	\[
	\rpz{\Psi}H\spz{\Psi} = \rpz{\Psi}\Hamout\spz{\Psi} \le O(\sqrt{\delta}).
	\]
	
	We write
	\[
	\spz{\Psi} = \frac{1}{\sqrt{T+1}} \sum_{t=0}^{T} \spz{\unary(t)}_{\clock} \otimes \spz{\psi_t}_{\state},
	\]
	where $\spz{\psi_t} = \Vvanilla_{[1\dotsc t]} \spz{\psi_{0}}$, and $\spz{\psi_0} = \spz{\phi}_{\witness} \otimes \spz{0^{2\log m + 1}}_{\ancilla}$.
	
	By the definition of $\Vvanilla$, we know that
	\[
	\spz{\psi_T} = \frac{1}{\sqrt{m}} \sum_{i \in [m]} (V_{\Pi_i} \spz{\psi} \spz{0})_{\data,\out} \spz{i}_{\idx}\spz{i}_{\midx}.
	\]
	
	By a straightforward calculation, we have that
	\begin{align*}
	\rpz{\Psi}\Hamout\spz{\Psi} &= \frac{1}{T+1} \cdot \rpz{\psi_T} (\proj{0}_{\out}) \spz{\psi_T} \\
								&= \frac{1}{T+1} \cdot \sum_{i \in [m]} \frac{1}{m} (V_{\Pi_i}^\dagger \rpz{\psi_T} \rpz{0})_{\data,\out} (\proj{0}_{\out}) (V_{\Pi_i} \spz{\psi_T} \spz{0})_{\data,\out}\\
								&= \frac{1}{T+1} \cdot \sum_{i \in [m]} \frac{1}{m} \rpz{\phi}\Pi_i\spz{\phi}.
	\end{align*}
	
	Hence, we have that
	\[
	\sum_{i \in [m]} \rpz{\phi}\Pi_i\spz{\phi} \le m \cdot O(\sqrt{\delta}).
	\]
	\end{proof}
	
	\begin{corollary}
		For a $(k,\eps)$-$\projLH$ instance $G = \sum_{i \in [m]} G_i$, let $H$ be the history Hamiltonian of the verifier $\Vvanilla$ with instance $G$. For a constant $\delta > 0$  that only depends on $k$ and $\eps$, we have
		\begin{itemize}
			\item $\lmin(G) = 0$ implies that $\lmin(H) = 0$.
			\item $\lmin(G) \ge \eps m$ implies that $\lmin(H) > \delta$.
		\end{itemize}
	\end{corollary}
	
	\subsubsection{Local verifier for $(k,\delta)$-$\History$-$\projLH$}\label{sec:van-local-estimation}
	
	From~\autoref{defi:history-Hamiltonians}, we have that 	
	\[
	H = \Hamout + \Hamprop + \Haminit + \Hamstab = \Hamout + \sum_{t \in [T]} \Hamprop_t + \sum_{i \in [B]} \Haminit_i + \sum_{t \in [T-1]} \Hamstab_t.
	\]
	by definition, it is easy to see that for the $M = 1 + T + B + (T-1) = 9$ summands above, only $\Hamprop_{T}$ is not at most $O(\log m)$-local. We have
	\begin{align*}
	\Hamprop_{T} &= \frac{1}{2} \left( \proj{10}_{\clock[T-1,T]} + \proj{1}_{\clock(T)} - U_{\sf test} \spz{1}\rpz{0}_{\clock(T)} - U_{\sf test}^\dagger \spz{0}\rpz{1}_{\clock(T)} \right). \\
	&= \sum_{i \in [m]} \frac{1}{2} \left( \proj{10}_{\clock[T-1,T]} + \proj{1}_{\clock(T)} - V_{\Pi_i} \spz{1}\rpz{0}_{\clock(T)} - V_{\Pi_i}^\dagger \spz{0}\rpz{1}_{\clock(T)} \right) \otimes \proj{i}_{\idx}.
	\end{align*}
	
	For each $i \in [m]$, we let
	\[
	\Hamprop_{T,i} = \frac{1}{2} \left( \proj{10}_{\clock[T-1,T]} + \proj{1}_{\clock(T)} - V_{\Pi_i} \spz{1}\rpz{0}_{\clock(T)} - V_{\Pi_i}^\dagger \spz{0}\rpz{1}_{\clock(T)} \right) \otimes \proj{i}_{\idx}.
	\]
	
	Note that $\Hamprop_{T,i}$ is now $O(\log m)$-local. Consider the following local verifier $\VHvanilla$ for $(k,\delta)$-$\History$-$\projLH$.
	
	\begin{construction}{The local verifier $\VHvanilla$ for $(k,\delta)$-$\History$-$\projLH$}
\begin{itemize}
	\item Given $\spz{\Phi} \in \Hclock \otimes \Hstate$. We first pick a uniform random term $J$ in $H$, with probability $1 - \frac{1}{M}$, $J \ne \Hamprop_{T}$, in this case we measure with POVM $\{J,I-J\}$, reject if the outcome is $J$.
	
	\item Otherwise, $J = \Hamprop_{T}$. In this case, we first measure $\idx$ to obtain $i \in [m]$, and then measure with POVM $\{ \Hamprop_{T,i}, I - \Hamprop_{T,i} \}$, reject if the outcome is $\Hamprop_{T,i}$.
	
	\item This verifier $\VHvanilla$ is local in the sense that it checks at most $O(\log m)$ qubits in the witness $\spz{\Phi}$.
\end{itemize}
	\end{construction}

	\begin{lemma}\label{lemma:van-local}
		$\VHvanilla$ rejects $\spz{\Phi} \in \Hclock \otimes \Hstate$ with probability exactly
		\[
		\frac{1}{M} \rpz{\Phi} H \spz{\Phi}.
		\]
	\end{lemma}
	\begin{proof}
		When $J \ne \Hamprop_{T}$, $\Avanilla$ rejects with probability $\rpz{\Phi} J \spz{\Phi}$.
		
		When $J = \Hamprop_{T}$, we write $\spz{\Phi} = \sum_{i=1}^{m} \sqrt{p_i} \spz{\eta_i}_{\sf other} \spz{i}_{\idx}$. We can see $\Avanilla$ rejects with probability
	\[
	\sum_{i=1}^{m} p_i \cdot \rpz{\eta_i} \Hamprop_{T,i} \spz{\eta_i}.
	\]
	
	We also have
	\[
	\rpz{\Phi}\Hamprop_{T}\spz{\Phi} = \sum_{i=1}^{m} p_i \cdot \rpz{\eta_i} \Hamprop_{T,i} \spz{\eta_i}
	\]
	as well.
	
	Hence, the overall procedure reject with probability
	\[
	\frac{1}{M} \rpz{\Phi} H \spz{\Phi}.
	\]
\end{proof}
\end{comment}

%\section{Encoded verifier and encoded history verifier}\label{sec:enc-verifier}

\begin{comment}
In this section we prove~\autoref{theo:history-problem-prop}, which is restated below.

\begin{reminder}{\autoref{theo:history-problem-prop}}
	For every $\eps > 0$, there is a constant $\delta > 0$ such that the followings hold for the $(k,\delta)$-$\History$-$\EncprojLH$ problem.
	\begin{itemize}
		\item (\textbf{Reduction from $(k,\eps)$-$\projLH$}) There is a reduction $\redEncH$ from $(k,\eps)$-$\projLH$ to $(k,\delta)$-$\History$-$\EncprojLH$, such that for a $(k,\eps)$-$\projLH$ instance $G$:
		\begin{itemize}
			\item $G \in (k,\eps)$-$\projLH_{\yes}$ implies $\redEncH(G) \in (k,\delta)$-$\History$-$\EncprojLH_{\yes}$.
			\item $G \in (k,\eps)$-$\projLH_{\no}$ implies $\redEncH(G) \in (k,\delta)$-$\History$-$\EncprojLH_{\no}$.
		\end{itemize}
  \item (\textbf{Simulation}) $(k,\delta)$-$\History$-$\EncprojLH$ is in $(2,O(\log m))$-$\SimQMA$ with completeness $1$ and soundness $1 - \Omega(\delta)$.
	\end{itemize}
\end{reminder}


We first introduce the following encoded version of $(k,\gamma)$-$\QSAT$.

\begin{construction}{$(k,\eps)$-$\EncprojLH$:}
	\begin{itemize}
		\item (\textbf{Input}) Given $m$ $kN$-local projections $\Pi^\Enc_{1},\dotsc,\Pi^\Enc_{m}$ acting on an $n \cdot N$-qubit register $\edata$, satisfying the following constraint:
		\begin{itemize}
			\item For each $i \in [m]$, there exists a $k$-local projection $\Pi_{i}$ acting on an $n$-qubit register $\data$ such that $\Pi^\Enc_{i} = \Enc(\Pi_i)$. Here, $\Enc(\Pi_i)$ denotes the projection to the encoding of the subspace $\Pi_i$ by $\Enc$.
		\end{itemize}
		
		Let $G^\Enc = \sum_{i \in [m]} \Pi^\Enc_i$. Decide between the following cases
		\begin{itemize}
			\item (\textbf{Yes}) $\lmin(G^\Enc) = 0$ or 
			\item (\textbf{No}) $\lmin(G^\Enc) \ge \eps m$.
		\end{itemize}
		
		\item For simplicity we always assume $\log m$ is an integer.
	\end{itemize}
\end{construction}

There is a striaghtforward reduction from $(k,\eps)$-$\projLH$ to $(k,\eps)$-$\EncprojLH$.

\begin{lemma}
	Given a $k$-local Hamiltonian $G = \sum_{i \in [m]} \Pi_i$ acting on $n$ qubits, where all $\Pi_i$'s are projections on $k$ qubits. Let $G^{\Enc} = \sum_{i \in [m]} \Enc(\Pi_i)$ acting on $n \cdot N$ qubits. It holds that $\lmin(G) = \lmin(G^{\Enc})$.
\end{lemma}
\cljnote{TODO: add a proof, which is pretty simple.}

==> succinct-tex <==

\section{A Candidate Succinct Argument for $\LocalQMA$ in $\QHROM$}\label{sec:succinct}

%\lnote{Here we only consider $\projLH$ and not the Gap-$\LH$... Perhaps need to say something}

In this section, we present a candidate succinct argument for $\LocalQMA$ in $\QHROM$. Assuming $\QPCP$, this succinct argument also works for all of $\QMA$.

\subsection{The Succinct Protocol $\Pisuc$}
\newcommand{\id}{\mathsf{id}}
\newcommand{\blk}{b}

\paragraph{Notation.} 

Let $L = (L_{\yes}, L_{\no}) \in (k,\gamma)\text{-}\LocalQMA_{s,c}$ for two integers $k,\gamma \in \N$ and two reals $s,c \in [0,1]$ such that $s < c$. Let $m_L$ and $p_L$ be the polynomials and $V_L$ be the $k$-local verifier in~\autoref{defi:localQMA}. Throughout this section, we will always use $n$ to denote the length of an input to $L$, $N = p_L(n)$ to denote the number of qubits in a witness for $V_L$, and $\lambda$ to denote the security parameter. 

We also set $\blk = \lambda /3$, and $\ell = N/\blk$. We assume that $\blk$ is an integer and $\ell$ is a power of $2$ for simplicity and without loss of generality since one can always add dummy qubits to the witness.

%Let $\lambda$ be the security parameter, $n = \lambda /3$, and $\ell = N/n$. We assume that $n$ is an integer and $\ell$ is a power of $2$ for simplicity. 

\paragraph*{The perfect binary tree $T_\ell$.} We will consider a perfect binary tree $T_\ell$ of $\ell$ leafs (see~\autoref{fig:binarytree} for an illustration). Note that $T_\ell$ has $\log\ell$ layers. We label the nodes in $T_\ell$ first from root to leaves and then from left to right, starting with $1$.

For a node $u$ in $T_\ell$, we observe that $u$'s parent is $\lfloor u/2 \rfloor$ if $u$ is not the root (\ie, $u \ne 1$) and $u$'s two children are $2u$ and $2u + 1$ if $u$ is not a leaf (\ie, $u < \ell$). We use $P_u$ to denote the set of nodes consisting of $u$ and all ancestors of $u$. Formally, we have
\[
P_u = \begin{cases}
\{u\} \quad& \text{if $u = 1$,}\\
\{u\} \cup P_{\lfloor u/2 \rfloor} \quad& \text{if $u > 1$.}
\end{cases}
\]

We also define $R_u$ as follows:
\[
R_u = \{\text{$u\in P_u$ or $\lfloor u/2\rfloor \in P$}  : u \in [2\ell - 1] \}.
\]
That is, a node $v$ belongs to $R_u$ if either $v$ is in $P_u$ or the parent of $v$ is in $P_u$. Also, for a set of node $S \subseteq [2\ell - 1]$, we set $R_S = \bigcup_{u \in S} R_u$.

\input{binarytree}

Given an $N$-qubit state $\sigma$, we define the following commitment algorithm (\autoref{algo:commit}) and the corresponding local decommitment algorithm (\autoref{algo:decommit}).

\begin{algorithm}[H]
	\caption{Algorithm for committing to an $N$-qubit quantum state}\label{algo:commit}
	\SetKwProg{Fn}{Function}{}{}
	\Fn{$\commit^{\caG}(\sigma,N,\lambda)$}{
		\KwIn{$\sigma$ is an $N$-qubit quantum state, $\lambda$ is the security parameter (recall that $\lambda = 3\blk$)}
		Let $\ell = N/\blk$\; %\tcp{We assume $\ell = 2^d$ for $d \in \N$ for simplicity}
		For each node $u$ in $T_\ell$, create a $\blk$-qubit register $\state^{(u)}$\;
		Store $\sigma$ in registers $\state^{(\ell)},\state^{(\ell+1)},\dotsc,\state^{(2\ell-1)}$\;
		\For{$u$ from $\ell - 1$ down to $1$}{
			Initialize $\state^{(u)}$ as $\spz{0^\blk}$\;
			Apply $\caG$ on $\state^{(2u)}$, $\state^{(2u+1)}$, and $\state^{(u)}$\;
		}
		\Return all qubits in $\{ \state^{(u)} \}_{u \in [2\ell - 1]}$\;
	}
\end{algorithm}

\begin{algorithm}[H]
	\caption{Algorithm for recovering part of the original quantum state}\label{algo:decommit}
	\SetKwProg{Fn}{Function}{}{}
	\Fn{$\decommit^{\caG^\dagger}(N,\lambda, S, \{ \eta_{u} \}_{u \in R_S})$}{
		\KwIn{$S \subseteq [2\ell - 1]$ is a subset of nodes in $T_\ell$, for each $u \in R_S$ $\eta_u$ is a $\blk$-qubit quantum state, $\lambda$ is the security parameter}
		Let $\ell = N/\blk$\; %\tcp{We assume $\ell = 2^d$ for $d \in \N$ for simplicity}
		For each node $u$ in $R_S$, create a $\blk$-qubit register $\state^{(u)}$, and store $\eta_u$ at $\state^{(u)}$\;
		\For{$u \in R_S \cap [\ell - 1]$, from smallest to the largest\label{line:order-decom}}{
			Apply $\caG^\dagger$ on $\state^{(2u)}$, $\state^{(2u+1)}$, and $\state^{(u)}$\;
			Measure $\state^{(u)}$ in the computational basis to obtain an outcome $z \in \bits^{\blk}$\;
			\lIf{$z \ne 0^{\blk}$}{\Return $\perp$}
		}
		\Return all qubits in $\{ \state^{(u)} \}_{u \in S}$\;
	}
\end{algorithm}

Finally, we are ready to specify the following candidate succinct argument for $L \in (k,\gamma)\text{-}\LocalQMA_{s,c}$.

\begin{construction}{The candidate succinct argument $\Pisuc$ for $L \in (k,\gamma)\text{-}\LocalQMA_{s,c}$}
	\begin{itemize}
		\item Both prover ($\caP$) and verifier ($\caV$) get access to a Haar random quantum unitary $\caG$ acting on $3\blk = \lambda$ qubits and its inverse $\caG^\dagger$. They also both get an input $x \in \bits^n$ to $L$. The goal for the prover is to convince the verifier that $x \in L_{\yes}$.
		
		%They both get an instance of $(k,\eps)$-$\projLH$ with Hamiltonian $G = \sum_{i \in [m]} \Pi_i$ acting on $N$ qubit. The goal is to determine whether $\lmin(G) = 0$ or $\lmin(G) \ge \eps \cdot m$, with the promise that one of them is the case. 
		
		Let $\ell = N/\blk$ and we assume that $\ell = 2^d$ for $d \in \N$.
		
		\item (\textbf{First message: $\caP \to \caV$}) The honest prover $\caP$ acts as follows: If $x \in L_{\no}$, $\caP$ aborts immediately. Otherwise, $\caP$ finds an $N$-qubit state $\sigma$ such that $V_L$ accepts with probability at least $c$, and runs $\commit(\sigma,N,\lambda)$ to obtain qubits $\{ \eta_{u} \}_{u \in [2\ell - 1]}$.
		
		$\caP$ then sends $\eta_{1}$ to $\caV$.
		
		\item (\textbf{Second message: $\caV \to \caP$}) $\caV$ now simulates the local verifier $V_L$. It first draws $i \getsR [m_L(n)]$ and sends $i$ to $\caP$, and then computes a $k$-size subset $S_i \subseteq [N]$ and a $\gamma$-size circuit $C_i$ acting on $k$ qubits.
		
		Let $W_i$ be the set of leaves in $T_\ell$ that contains the qubits indexed by $S_i$. That is,
		\[
		W_i = \{ \ell + \lfloor (u-1)/\blk \rfloor : u \in S_i \}.
		\]
		
		\item (\textbf{Third message: $\caP \to \caV$}) The honest prover $\caP$ sends $\{\eta_u\}_{u \in R_{W_i}, u \ne 1}$ to $\caV$. $\caV$ then runs $\decommit(N,\lambda,W_i,\{ \eta_u \}_{u \in R_{W_{i}}})$ (note that $\caV$ already has $\eta_1$). If $\decommit$ returns $\perp$, $\caV$ rejects immediately.
		
		Otherwise, $\caV$ continues the simulation of $V_L$ by running $C_i$ using $\{ \eta_{u} \}_{u \in W_i}$, and $\caV$ accepts if and only if $V_L$ accepts.
	\end{itemize}
\end{construction}

\subsection{Analysis of $\Pisuc$}

Now we prove the completeness and succinctness of $\Pisuc$.

\begin{theorem}\label{theo:Pisuc-c-and-s}
	Let $\Pisuc$ be the protocol between $\caP$ and $\caV$ for the promise language $L \in (k,\gamma)\text{-}\LocalQMA_{s,c}$. For every $x \in \bits^n$, the following hold:
	\begin{description}
		\item[] \textbf{Completeness:}
		{ 	If $x \in L_{\sf yes}$, then for every $\caG \in \Haar(2^\lambda)$,
			\[
			\Pr[(\caV^{\caG,\caG^\dagger} \leftrightarrows \caP^{\caG,\caG^\dagger} )(x) = 1] \ge c.
			\]}
		\item[]  \textbf{Succinctness:} {
			$\caP$ and $\caV$ communicate at most $O(k \cdot \log n \cdot \lambda)$ qubits in total. }
		
		\item[] \textbf{Efficiency:} {$\caV$ runs in $\poly(n,k,\gamma)$ time. If $V_L$ is strongly explicit, then $\caV$ runs in $O(k \cdot \log n \cdot \lambda + \poly(\log n,k,\gamma))$ time.
		}
	\end{description}
\end{theorem}
\begin{proof}
	We first establish the succinctness part. Examining the protocol $\Pisuc$, one can see that the first message takes $O(\lambda)$ qubits, the second messages takes $O(\log m_L(n)) = O(\log n)$ classical bits, and the third message takes $O\left( |R_{W_i}| \cdot \lambda \right)$ qubits. Note that $|R_{W_i}| \le |W_i| \cdot O(\log \ell) \le k \cdot O(\log N) \le O(k \cdot \log n)$, the total communication complexity is thus bounded by $O(k \cdot \log n \cdot \lambda)$. 
	
	For the running time of $\caV$, one can see that its running time is dominated by the running time of $\decommit(N,\lambda,W_i,\{ \eta_u \}_{u \in R_{W_i}})$ and the running time of $V_L$ computing $W_i$ and $C_i$, which are at most $O(k \cdot \log N \cdot \lambda)$ and $\poly(n,k,\gamma)$ ($\poly(\log n,k,\gamma)$ if $V_L$ is strongly explicit), respectively.
	
	Now we prove the completeness. Let $\caG_{(u)}$ be a $\caG$ gate applying on registers $\state^{(2u)}$, $\state^{(2u+1)}$, and $\state^{(u)}$. Then we know for the honest prover $\caP$, when $x \in L_{\yes}$, it prepares an $N$-qubit state $\sigma$ that makes $V_L$ accepts with probability at least $c$, and then applies $U_{\sf com} \coloneqq \caG_{(\ell-1)} \cdot \dotsc\cdot\caG_{(1)}$ to $\sigma \otimes \proj{0}_{\state^{(1)},\dotsc,\state^{(\ell-1)}}$.
	
	Let $U_{\sf decom} \coloneqq U_{\sf com}^{\dagger} = \caG_{(1)}^\dagger\cdot \dotsc \cdot \caG_{(\ell-1)}^\dagger$. Recall that verifier $\caV$ at the end simulates the quantum circuit $C_i$ only on registers in $\{ \state^{(u)} \}_{u \in W_i}$. We now argue that $\caV$ is effectively simulating $C_i$ on
	\[
	U_{\sf decom}^{\dagger} U_{\sf com} \sigma \otimes \proj{0}_{\state^{(1)},\dotsc,\state^{(\ell-1)}} = \sigma \otimes \proj{0}_{\state^{(1)},\dotsc,\state^{(\ell-1)}}.
	\]
	
	The reason is that $\decommit(N,\lambda,W_i,\{ \eta_u \}_{u \in R_{W_i}})$ performs all gates in $U_{\sf decom}$ that lies in the lightcone of the registers $\{ \state^{(u)} \}_{u \in W_i}$ in the chronological order (see Line~\ref{line:order-decom} of \autoref{algo:decommit}). Also, since $\caP$ starts with the state $\sigma \otimes \proj{0}_{\state^{(1)},\dotsc,\state^{(\ell-1)}}$, $\decommit$ never outputs $\bot$. Therefore, $\caV$ is simulating $V_L$ faithfully on $\sigma$, meaning that it accepts with probability at least $c$.
\end{proof}

We conjecture that the soundness also holds.
\begin{conjecture}[$\Pisuc$ is sound in $\QHROM$]\label{conj:soundness}
	Let $\Pisuc$ be the protocol between $\caP$ and $\caV$ for the promise language $L \in (k,\gamma)\text{-}\LocalQMA_{s,c}$. For every $x \in \bits^n$, the following hold:
	\begin{description}
		\item[] \textbf{Soundness:}
		{ 
			If $x \in L_{\no}$, then for every $t \in \N$ and all (potentially malicious) $\caP^*$ that makes at most $t$ total queries to $\caG$ and $\caG^\dagger$, for some $\delta = \delta(t,\lambda) = \poly(t)/2^{\Omega(\lambda)}$, it holds that
			\[
			\Pr_{\caG \getsR \Haar(2^\lambda)} \left[ \Pr[(\caV^{\caG,\caG^\dagger}  \leftrightarrows (\caP^*)^{\caG,\caG^\dagger} ) (x) = 1)] \ge s + \delta \right] \le \delta.
			\]
		}
	\end{description}
\end{conjecture}

\subsection{Discussions}\label{sec:suc-discussions}

We remark that (1) the constant soundness in \autoref{conj:soundness} and the constant completeness in~\autoref{theo:Pisuc-c-and-s} can be easily amplified to $n^{-\omega(1)}$ and $1-n^{-\omega(1)}$ by repeating the protocols $\log^2 n$ times, and (2) assuming $\QPCP$, the protocol works for all languages in $\QMA$.

\begin{corollary}\label{cor:suc-protocol-for-LocalQMA}
	Assuming \autoref{conj:soundness}, there is a protocol for $L \in (k,\gamma)\text{-}\LocalQMA_{s,c}$ with $\lambda \cdot \polylog(n)$ communication complexity, completeness $1-n^{-\omega(1)}$ and soundness $n^{-\omega(1)}$ in $\QHROM$. Also, if $V_L$ is strongly explicit, then the verifier running time of the protocol is also bounded by $\lambda \cdot \polylog(n)$.
	
	Moreover, if we further assume that $\QPCP$ holds, then the aforementioned succinct protocol exists for every $L \in \QMA$.
\end{corollary}

Moreover, we suspect that if we apply $\Pisuc$ to $\SimQMA$\footnote{The prover first commits to a state $\sigma$ and sends $\state^{(1)}$ to the verifier; the verifier then simulates the local verifier $V_L$ for $L \in \SimQMA$ by asking the prover to open relevant qubits in $\sigma$; this simulation requires $\ell$ rounds between the prover and the verifier if $V_L$ is $\ell$-adaptive.} instead of $\LocalQMA$, the resulting protocol would be both succinct and zero-knowledge.\footnote{A candidate simulator first guesses the sequence $\tau_0,\dotsc,\tau_\ell$, and then simulates the protocol with the state $(\sigma') \otimes I_{\bar{S}}$, where $\sigma'$ and $S$ are from~\autoref{defi:simQMA}, and restarts if the simulated run does not give the same sequence $\tau_0,\dotsc,\tau_\ell$. See also~\autoref{sec:zk-proof-of-zk}.} We leave this as an interesting open question.

Another open question is whether we can instantiate the protocol $\Pisuc$ in the more standard $\QROM$. A natural way to do this is to simulate a Haar random unitary by a standard random oracle; see~\cite[Section~6]{JiL018} for some candidate constructions. 

% Emm... actually it just seems true, perhaps I should try to prove it later when I have time...

\begin{comment}

\subsection{Discussions on soundness for the depth-$2$ case}

In this subsection we discuss the soundness of $\Pisuc$ when $\ell = N/n = 2$. See below for a formal definition of (potentially malicious) prover $\caP$'s strategy by $t$-query quantum algorithms.

\begin{construction}{Special case of $\Pisuc$ when $\ell = 2$ for $(k,\eps)$-$\projLH$}
\begin{itemize}
\item Both prover ($\caP$) and verifier ($\caV$) get access to a Haar random quantum unitary $\caG$ acting on $3n$ qubits. They both get an instance of $(k,\eps)$-$\projLH$ with Hamiltonian $G = \sum_{i \in [m]} \Pi_i$ acting on $2n$ qubit. The goal is to determine whether $\lmin(G) = 0$ or $\lmin(G) \ge \eps \cdot m$, with the promise that one of them is the case.

\item Prover's strategies are formulated by bounded-query quantum algorithms. A $t$-query quantum algorithm here is an arbitrary size quantum circuit in which the total number of $\caG$ and $\caG^\dagger$ gates (these gates can act on any $3n$ qubits) is at most $t$. Note that the circuit of prover's quantum algorithm depends on the instances $G = \sum_{i \in [m]} \Pi_i$, but not on the random Haar unitary $\caG$, which is unknown in advance.

\item There are three registers: a $2n$-qubit register $\state$, an $n$-qubit register $\com$ and an ancilla register $\ancilla$ that can contain any number of qubits.

\item In the first round, $\caP$ applies a $t$-query unitary $W$ acting on $\Hstate \otimes \Hcom \otimes \Hancilla$. We let $\spz{\Phi} = W \spz{0}_{\state,\com,\ancilla}$. $\caP$ then sends the $\com$ register to $\caV$.

\item In the second round, $\caV$ picks a random integer $i \in [m]$ and sends it to $\caP$ (as a classic string).

\item In the third round, $\caP$ applies a $t$-query unitary $V_i$ acting on $\Hstate \otimes \Hancilla$ based on the message from the $\caV$. $\caP$ then sends the register $\Hstate$ to $\caV$.

\item Finally, $\caV$ applies $\caG^\dagger$ to $\Hstate \otimes \Hcom$ and get a mixed state $\sigma$ on $\Hstate \otimes \Hcom$. It then measures $\com$ and rejects if the outcome is not $0^{n}$. Next it measures $\{ \Pi_i,I-\Pi_i \}$ on $\Hstate$ and rejects if the outcome is $\Pi_i$.
\end{itemize}
\end{construction}

In the following we will assume that a malicious prover $\caP$ can make the honest verifier $\caV$ accepts a no instance with high probability. We will see $\caP$ needs to be able to ``switch commitment'' in a formal sense.

Formally, assume that $\lmin(G) > \eps m$ and yet there are $t$-query algorithms $W$ and $\{V_i\}_{i \in [m]}$ making $\caV$ accepts with probability $1-\delta$ over both the randomness of $\caG$ and $\caV$, where $\delta > 0$ is a small constant to be fixed later.

Let $\spz{\Phi_i} =  (\caG^\dagger \otimes I_\ancilla) \cdot (V_i \otimes I_{\com}) \spz{\Phi}$ be the final state of the whole system before its measurements on $\com$ and $\state$, when $\caV$ sends $i$ to $\caP$. Note that $\spz{\Phi}$ also includes qubits in $\ancilla$, while $\caV$ does not have them.

Since $\caV$ rejects with probability at most $\delta$.

By a simple Markov inequality, the following holds. (Note that $\caV$ rejects if either the valid check on $\com$ fails or the measurement on $\state$ has outcome $\Pi_i$.)
\begin{claim}\label{claim:phi_i}
For a $1-\sqrt{\delta}$ fraction of $i \in [m]$, we know that there exists $\phi_i$ on $\state$ such that
\[
\left\| \Tr_{\ancilla}(\proj{\Phi_i}) - \phi_i \otimes \proj{0^n}_\com \right\|\le \sqrt{\delta},
\]
and
\[
\Tr[\phi_i \Pi_i] \le \sqrt{\delta}.
\]
We say those $i$'s are good.
\end{claim}

For each $i \in [m]$, if $i$ is good, then we let $\phi_i$ be the corresponding density matrix in~\autoref{claim:phi_i}. Otherwise, we simply let $\phi_i$ be $\proj{0}_{\state}$.

Since $\lmin(G) > \eps m$, we know that $\Tr[G \phi_i] > \eps m$. Summing up for all $i \in [m]$, we have
\[
\sum_{i \in [m]} \sum_{j \in [m]} \Tr[\phi_i \Pi_j] > \eps \cdot m^2.
\]

In particular, there must exist two distinct good $a,b \in [m]$ such that $\Tr[\phi_a \Pi_b] \ge \eps / 2$ (since $\delta$ is small enough), which means $\| \phi_a - \phi_b \|_\tr \ge \eps / 3$.


Now we will focus on these two good $a,b \in [m]$.

Hence, we end up with
\[
\left\| \left[ \caG^\dagger V_i W \proj{0} W^\dagger V_i^\dagger \caG \right]_{\state,\com} - \phi_i \otimes \proj{0^n}_\com \right\|\le \sqrt{\delta}\quad\text{ for $i \in \{a,b\}$} \quad\text{and}\quad \| \phi_a - \phi_b \| \ge \eps / 3.
\]

Letting $U_1 = \caG^\dagger V_a W$ and $U_2 = V_bV_a^\dagger$, they both take at most $2t + 2$ queries. And we have that for some density matrices $\phi_1,\phi_2$ on $\state$, we have that
\[
\left\| (U_1\proj{0}U_1^\dagger)_{\state,\com}  - \phi_1 \otimes \proj{0^n}_\com \right\| \le \sqrt{\delta} \quad\text{and}\quad 
\left\| ( \caG^\dagger U_2 \caG U_1\proj{0}U_1^\dagger \caG^\dagger U_2 \caG)_{\state,\com}  - \phi_2 \otimes \proj{0^n}_\com \right\| \le \sqrt{\delta}
\]
where $U_2$ only acts on $\ancilla$ and $\state$, and
\[
\| \phi_1 - \phi_2 \| \ge \eps / 3.
\]

We conjecture that the above should only happen with very small probability over the choice of $\caG$.
% RELEVANT --RM

\begin{conjecture}
For every two $t$-query quantum random algorithms $U_1,U_2$ such that $U_1$ acts on $\state,\com,\ancilla$ and $U_2$ only acts on $\state,\ancilla$. Let $\Pi$ be the projector to space $\Hstate \otimes \proj{0}_\com$, and
\[
\spz{\psi_1} = U_1 \spz{0}_{\state,\com,\ancilla}\quad\text{and}\quad \spz{\psi_2} =  (\caG^\dagger \otimes I_\ancilla) (U_2 \otimes I_\com) (\caG \otimes I_\ancilla)\spz{\psi_1}
\]
the following happens with very small probability over $\caG$:
\begin{itemize}
\item $\Tr[\Pi \psi_1] \ge 1-\kappa_1$, $\Tr[\Pi \psi_2] \ge 1 - \kappa_1$ and $\|(\psi_1)_{\state,\com} - (\psi_2)_{\state,\com}\| \ge \kappa_2$, where $\kappa_1,\kappa_2$ are two parameters to be chosen later.
\end{itemize}
\end{conjecture}

Note that the the conditions on $\spz{\psi_1}$ and $\spz{\psi_2}$ imply that
\[
(\caG \otimes I_\ancilla)  \spz{\psi_2} = (U_2 \otimes I_\com) (\caG \otimes I_\ancilla)  \spz{\psi_1}.
\]
Also, $\spz{\psi_1}$ and $\spz{\psi_2}$ are close to two states before commitment (their restriction on $\com$ is close to $\spz{0^n}$). 

The above conjecture basically says that there is no way of (approximately) finding two quantum states $(\sigma_1)_{\state} \otimes \proj{0^n}_\com$ and $(\sigma_2)_\state \otimes \proj{0^n}_\com$ such that $\sigma_1$ and $\sigma_2$ are distinguishable ($\kappa_2$ away), and one can transform between the below two commitments
\[
\caG ((\sigma_1)_{\state} \otimes \proj{0^n}_\com)
\]
and
\[
\caG ((\sigma_2)_{\state} \otimes \proj{0^n}_\com)
\]
by only acting on $\state$.

\subsection{A proof for special case}

\begin{theorem}
For every $t$-query quantum random algorithms $U$ such that $U$ only acts on $\state$. The following happen with very small probability: $\caG (\spz{0}_\state \spz{0}_\com)$ has trace distance $\delta$ to $U \caG (\spz{1}_\state \spz{0}_\com)$.
\end{theorem}

\begin{proof}
Let $\caD$ be a pseudorandom state distribution
\end{proof}
\end{comment}



==> zero-knowledge-tex <==
\section{Zero-Knowledge Protocols from Locally Simulatable Proofs}\label{sec:zk}

In this section, we give a general construction of zero-knowledge proofs for all problems in $(k,\ell)$-$\SimQMA$. Our protocol generalizes the zero-knowledge protocol for $(k,1)$-$\SimQMA$ in~\cite{BroadbentG20}. Since the locally simulatable verifier in $(k,\ell)$-$\SimQMA$ is adaptive when $\ell > 1$, our analysis is more involved than that of~\cite{BroadbentG20}.


\subsection{Commitment Schemes}

To construct our zero-knowledge proof system, we will need commitment schemes that are
unconditionally binding and computationally hiding. We now present the formal definition of such schemes. Our definitions are borrowed from~\cite{ChiaCY21}.

%%%%%commitment%%%%%%%%%%%%%
\newcommand{\Exp}{\mathsf{Exp}}
\newcommand{\pp}{\mathsf{pp}}
%\newcommand{\com}{\mathsf{com}}
%\newcommand{\commit}{\mathtt{com}}
%\newcommand{\open}{\mathtt{open}}
\newcommand{\Com}{\mathsf{Com}}
\newcommand{\CBCom}{\mathsf{CBCom}}
\newcommand{\Gen}{\mathsf{Gen}}
\newcommand{\Setup}{\mathsf{Setup}}
\newcommand{\Commit}{\mathsf{Commit}}
\newcommand{\ComGen}{\Com.\mathsf{Gen}}
\newcommand{\ComSetup}{\Com.\mathsf{Setup}}
\newcommand{\ComCommit}{\Com.\mathsf{Commit}}
\newcommand{\CBSetup}{\CBCom.\mathsf{Setup}}
\newcommand{\CBGen}{\CBCom.\mathsf{Gen}}
\newcommand{\CBCommit}{\CBCom.\mathsf{Commit}}
\newcommand{\SBCom}{\mathsf{SBCom}}
\newcommand{\SBSetup}{\SBCom.\mathsf{Setup}}
\newcommand{\SBCommit}{\SBCom.\mathsf{Commit}}
\newcommand{\SBSetupSigma}{\SBCom_\Sigma.\mathsf{Setup}}
\newcommand{\SBCommitSigma}{\SBCom_\Sigma.\mathsf{Commit}}
%\newcommand{\ck}{\mathsf{ck}}
\newcommand{\ch}{\mathsf{ch}}
\newcommand{\chspace}{\mathcal{C}\mathcal{H}}
\newcommand{\COM}{\mathcal{C}\mathcal{O}\mathcal{M}}
\newcommand{\ppspace}{\mathcal{PP}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\hiding}{\mathsf{hiding}}
\newcommand{\binding}{\mathsf{binding}}
\newcommand{\clbinding}{\mathsf{cl}\text{-}\binding}
\newcommand{\rand}{\mathsf{rand}}
\newcommand{\randspace}{\calR}
\newcommand{\OUT}{\mathsf{OUT}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\secpar}{\lambda}
\newcommand{\sample}{\getsR}
\newcommand{\A}{\caA}

\begin{definition}[Commitment.]\label{def:commitment}
	A (two-message) commitment scheme   with message space $\calM$, randomness space $\calR$, commitment space $\COM$, and a public parameter space $\ppspace$  consists of two classical PPT algorithms $(\Setup,\Commit)$:
	\begin{description}
		\item[$\Setup(1^\secpar)$:] The setup algorithm takes the security parameter $1^\secpar$ as input and outputs a public parameter $\pp\in \ppspace$.
		\item[$\Commit(\pp,m)$:] The committing algorithm takes a public parameter $\pp\in \ppspace$ and a message $m\in \calM$ as input and outputs a commitment $\com\in \COM$. 
	\end{description}
	We say that a commitment scheme is \emph{non-interactive} if a public parameter $\pp$ generated by $\Setup(1^\secpar)$ is always just the security parameter $1^\secpar$. For such a scheme, we omit to write $\Setup$.
	
	We define the following security notions for a commitment scheme.
	
	\paragraph{Statistical/Computational Hiding.}
	For an adversary $\A$, we consider an experiment $\Exp_{\A}^{\hiding}(1^\secpar)$ defined below:
	\begin{enumerate}
		\item $\A$ is given the security parameter $1^\secpar$ and sends a (possibly malformed) public parameter $\pp\in\ppspace$ and $(m_0,m_1)\in \calM^2$ to the challenger %and a (possibly quantum) state $\st_\A$.
		\item The challenger randomly picks $b\sample \bits$, computes $\com\sample \Commit(\pp,m_b)$, and sends $\com$ to $\A$. 
		\item $\A$ is given a commitment $\com$ and outputs $b'\in \bits$.
		The experiment outputs $1$ if $b=b'$ and $0$ otherwise.
	\end{enumerate}
	We say that a commitment scheme satisfies statistical (resp. computational) hiding if for any unbounded-time (resp. non-uniform QPT) adversary $\A$, we have
	\begin{align*}
	|\Pr[1\sample \Exp_{\A}^{\hiding}(1^\secpar)]-1/2|=\negl(\secpar).
	\end{align*}
	\begin{remark}\label{remark:rec-run-setup}
		Our definition of hiding requires that the security should hold even if $\pp$ is maliciously generated. Thus, the hiding property holds even if a receiver runs the setup algorithm. 
	\end{remark}
	
	
	\paragraph{Perfect/Statistical/Computational Binding.}
	We say that a non-interactive commitment scheme satisfies statistical (resp. computational) binding if for any unbounded-time (resp. non-uniform QPT) adversary $\A$, we have  
	\begin{align*}
	\Pr[\Commit(\pp,m;r)=\Commit(\pp,m';r')\land m\neq m' : \pp \sample \Setup(1^\secpar),(m,m',r,r')\sample \A(\pp)]=\negl(\secpar).
	\end{align*}
	We say that a scheme satisfies perfect binding if the above probability is $0$ for all unbounded-time adversary $\A$.
\end{definition}

\paragraph{Instantiations.}
A computationally hiding and statistically binding commitment scheme exists under the existence of post-quantum one-way functions \cite{Naor91,HastadILL99} (see also~\cite{ChiaCY21}). A computationally hiding and perfectly binding non-interactive commitment scheme exists under the QLWE assumption \cite{GoyalHKW17, Lombardi19}.

\subsection{Computational Zero-knowledge Proofs for $(k,\ell)$-$\SimQMA$}

For a $q$-qubit quantum state $\sigma$ and two strings $a,b \in \bits^q$, we define 
\[
\tilde{\sigma}_{a,b} = X^{a} Z^{b} \sigma Z^{b} X^{a}.
\]

Now we define our protocol $\Pizk$.

\begin{construction}{Zero Knowledge Protocol $\Pizk$ for $(k,\ell)$-$\SimQMA$}
	\begin{enumerate}
		\item (\textbf{Set up}) Let $L = (L_{\yes},L_{\no}) \in (\ell,k)\text{-}\SimQMA$ and $V_L$ be the corresponding $\ell$-adaptive verifier. Let $x \in L$, $n = |x|$, functions $p,m,c$ and $s$ be as in~\autoref{defi:simQMA}. 
		
		\item The honest prover $\caP$ aborts immediately if $x \in L_{\no}$. Otherwise, let $\sigma$ be the simulatable witness of $V_L$. $\caP$ picks $a,b \getsR \bits^{p(n)}$ and $r \getsR \caR$, where $\caR$ is all of the possible randomness needed to commit to $2 p(n)$ bits with the security parameter $\lambda$ set to $n$.
		
		\item $\caP$ sends $\tdsigma_{a,b} \otimes \proj{\comm^r_{a,b}}$ to $\caV$, where $\comm^r_{a,b}$ is the commitment to each bit of $a,b$, with randomness $r$.
		
		\item The honest verifier $\caV$ simulates the verifier $V_L$ as follows:
		\begin{enumerate}
			\item $V_L$ first draws $\tau_0 \getsR [m(n)]$. Recall that we use $\tau_i$ to denote the outcome obtained by $V_L$ in the $i$-th round, and $\tau_{\le i} = (\tau_0,\dotsc,\tau_i)$. 
			
			\item At the beginning of the $i$-th round, $V_L$ computes a subset $S_i = S_i(\tau_{\le i-1})$ with $ |S_i| \le k$.
			
			\item $\caV$ sends $\tau_{i-1}$ to $\caP$. $\caP$ computes $S_i$ and opens the commitment for $a_{|S_i}$ and $b_{|S_i}$. $\caV$ rejects immediately if any of the commitments does not open.
			
			\item $\caV$ now first decommits the qubits in $S_i$ by applying $Z^{b_{|S_i}} X^{a_{|S_i}}$ to the corresponding qubits in $\tdsigma_{a,b}$, and then simulates $V_L$ to perform the POVM $\{ \Pi_j \}_{j \in [m(n)]}$ and records $\tau_i$ accordingly.
			
			\item Finally, at the end of $\ell$-th round, $\caV$ accepts iff $V_{L}$ accepts.
		\end{enumerate}
	\end{enumerate}
\end{construction}

In the following, we show that using a non-interactive computationally hiding and perfectly binding commitment scheme in $\Pizk$ makes it a quantum computational zero-knowledge proof system with the same correctness and soundness as the corresponding $(k,\ell)$-$\SimQMA$ language. See~\autoref{sec:generalizations} for discussions on other instantiations of $\Pizk$.

We need the following two lemmas.

\begin{lemma}\label{lemma:c-and-s}
	$\Pizk$ instantiated with a non-interactive computationally hiding and perfectly binding commitment scheme has completeness $c(n)$ and soundness $s(n)$.
\end{lemma}

\begin{lemma}\label{lemma:zero-knowledge}
	Assuming $\ell = O(1)$ and $k = O(\log n)$, $\Pizk$ instantiated with a non-interactive computationally hiding and perfectly binding commitment scheme is computational zero-knowledge.
\end{lemma}

Hence, the following theorem follows immediately from the two lemmas above.

\begin{theorem}
	Under the QLWE assumption, there is a constant-round computational zero-knowledge proof system with soundness $s(n)$ and completeness $c(n)$ for $(O(\log n),O(1))$-$\SimQMA_{s(n),c(n)}$.
\end{theorem}

We will prove~\autoref{lemma:c-and-s} and~\autoref{lemma:zero-knowledge} separately.

\subsubsection{Proof of~\autoref{lemma:c-and-s}}

We first prove~\autoref{lemma:c-and-s}.

\begin{proofof}{\autoref{lemma:c-and-s}}\item
	\paragraph*{Completeness.} By~\autoref{defi:simQMA}, if $x \in L_{\yes}$, the honest prover $\caP$ can simply follow the protocol with a proof $\sigma$ that makes $V_L$ accepts with probability at least $c(n)$. Since the honest verifier $\caV$ simulates $V_L$ faithfully, the acceptance probability of $\caV$ is also at least $c(n)$.
	
	\paragraph*{Soundness.} Next, we assume $x \in L_{\no}$ and analyze the soundness of the protocol. Let $\psi \otimes \proj{z}$ be the state sent by $\caP$ in the first round, where $\psi$ is supposed to be a $p(n)$-qubit proof for the $(k,\ell)$-$\SimQMA$ problem $L$, and $z$ is the classical commitment to one-time pad key $a$ and $b$. Note that we can, without loss of generality, assume $\spz{z}$ is a classical value since $\caV$ can measure $z$ in the computational basis first and $\caP$ can send the $z$ that maximizes the acceptance probability.
	
	For a similar reason, we can also assume during the simulation of $V_{L}$ by $\caV$, the prover $\caP$ replies classical bits for all rounds.
	
	Since the commitment scheme is perfectly binding, we can define two unique strings $a,b \in \bits^{p(n)}$ from $z$, such that the committed $2p(n)$ bits can only be opened according to $a$ and $b$ (if the commitment allows no opening, we set that bit to be $0$).
	
	Since $\caV$ rejects immediately when $\caP$ fails to open the corresponding bits, the acceptance probability of $\caV$ is at most the acceptance probability of $V_L$ on the state $ Z^{b} X^{a} \psi X^a Z^b$. Since $x \in L_{\sf no}$, the acceptance probability is thus at most $s(n)$.
\end{proofof}

\subsubsection{Proof of~\autoref{lemma:zero-knowledge}}\label{sec:zk-proof-of-zk}

%Our proof below essentially follows the proof of~\cite[Lemma~5.3]{BroadbentG20}, with some crucial modifications to address the difference that now our simulatable verifier $V_L$ can be adaptive.

In the following, we prove~\autoref{lemma:zero-knowledge}. We will always assume $\ell = O(1)$, $k = O(\log n)$, and the security parameter $\lambda$ for the commitment scheme is set to the input length $n$. We first define the following simulator $\caS$.

\newcommand{\rcom}{r}
\newcommand{\hatV}{\widehat{V}}
\newcommand{\btau}{\bar{\tau}}

\begin{construction}{Simulator $\caS$ for $\Pizk$ for a malicious verifier $\hatV$ with side-information $\xi$}
	\begin{enumerate}
		\item (\textbf{Set up}) Let $L = (L_{\yes},L_{\no}) \in (\ell,k)\text{-}\SimQMA$ and $V_L$ be the corresponding $\ell$-adaptive verifier. Let $x \in L$, $n = |x|$, functions $p,m,c$ and $s$ be as in~\autoref{defi:simQMA}. Let $\sigma$ be the simulatable witness of $V_L$ given input $x$.
		
		\item $\caS$ picks $\btau_0, \btau_1,\dotsc,\btau_{\ell}$ as $\ell + 1$ i.i.d. samples from the uniform distribution over $[m(n)]$, $a,b \getsR \bits^{p(n)}$ and $\rcom \getsR \caR$. Recall that $\btau_{\le i}$ denotes $\btau_0,\dotsc,\btau_i$. For simplicity, we will also use $\btau$ and $m$ to denote $\btau_{\le \ell}$ and $m(n)$, respectively.
		
		\item Let $S_1,\dotsc,S_\ell$ be the corresponding set of $V_L$ given the sequence $\btau_{\le \ell}$ and let $S = \bigsqcup_{i \in [\ell]} S_i$. $\caS$ create the state
		\[
		\Psi = \tilde{\sigma}^{\btau}_{a,b} \otimes \proj{\comm^{\rcom}_{a,b}} \otimes \xi,
		\]
		where $\sigma^{\btau} = \sigma' \otimes \proj{0}_{[p(n)] \setminus S}$, and $\sigma'$ is density matrix on $S$ that can be computed in $\poly(n,2^{|S|}) = \poly(n,2^{\ell k})$ time given $x$ and $\btau$ from~\autoref{defi:simQMA}.
		
		\item $\caS$ runs $\hatV$ with $\Psi$ to obtain the simulated sequence $\tau_0,\dotsc,\tau_\ell$, and aborts immediately if they are not equal to the guessed sequence $\btau_0,\btau_1,\dotsc,\btau_\ell$.
	\end{enumerate}
\end{construction}

\newcommand{\Msg}{\mathsf{Msg}}
\newcommand{\Open}{\mathsf{open}}
\renewcommand{\COM}{\mathsf{COM}}
\newcommand{\Opens}{\mathsf{Opens}}

We set
\[
\COM^{r}_{a,b} \coloneqq \proj{\comm^{\rcom}_{a,b}}.
\]

For a sequence $\tau_{\le i} \in [m]^{i+1}$, we define
\[
\Opens^{\tau_{\le i}}_{a,b,r} \coloneqq \bigotimes_{j=0}^{j=i} \proj{\Open_{a,b,r}^{\tau_{\le j}}},
\]
where $\Open_{a,b,r}^{\tau_{\le j}}$ is the unique opening for the set $S_{j+1}$ (that can be computed from the input $x$ and $\tau_{\le j}$). Note that if $j = \ell$, then $\Open_{a,b,r}^{\tau_{\le j}} = 0$, since there is no set $S_{\ell + 1}$.

Next, we set up some notation to simplify the analysis of the simulator $\caS$.

\paragraph*{Intermediate states when running $\hatV$ on the simulatable witness $\sigma$.} We can assume that $\hatV$ proceeds in $\ell+1$ phase, and we use $\hatV_{0},\dotsc,\hatV_{\ell}$ to denote these $\ell + 1$ phases.

In the beginning, after the honest prover $\caP$ sends her first message, $\hatV$ sees
\[
\Phi = \sum_{a,b,r} \tilde{\sigma}_{a,b} \otimes \COM^r_{a,b} \otimes \xi,
\]
where $\xi$ is the side-information of $\hatV$, and $\sigma$ is the simulatable witness for $V_L$ given the input $x$.

Next, $\hatV$ applies $\hatV_0$ to the state above, since classical information can be copied, we can assume it acts as follows
\begin{align*}
&\hatV_0 \sum_{a,b,r} \tilde{\sigma}_{a,b} \otimes \COM^r_{a,b} \otimes \xi \hatV_0^\dagger\\
= &\sum_{\tau_0} p_{\sigma,a,b,r,\tau_0} \phi_{\sigma,a,b,r,\tau_0} \otimes \COM^r_{a,b} \otimes \proj{\tau_0}.
\end{align*}

After that, since the honest prover $\caP$ sends back the classical string $\Open_{a,b,r}^{\tau_0}$, the state becomes
\[
\sum_{\tau_0} p_{\sigma,a,b,r,\tau_0} \phi_{\sigma,a,b,r,\tau_0} \otimes \COM^r_{a,b} \otimes \proj{\tau_0} \otimes \Opens_{a,b,r}^{\tau_{\le 0}}.
\]

Again, the verifier now applies $\hatV_{1}$, which gives $\tau_1$, and the prover responds by $\Open_{a,b,r}^{\tau_{\le 1}}$. Continuing this way, the state of $\hatV$ at the end of round $i$, denoted by $\Phi_i$, can be written as (we denote the first round by round $0$ to make notation consistent)
\[
\Phi_i \coloneqq \sum_{\tau_{\le i}} p_{\sigma,a,b,r,\tau_{\le i}} \phi_{\sigma,a,b,r,\tau_{\le i}} \otimes \COM^r_{a,b} \otimes \proj{\tau_{\le i}} \otimes \Opens_{a,b,r}^{\tau_{\le i}}.
\]

We also set $\Phi_{-1} = \Phi$ for convenience.


\paragraph*{Intermediate states when running the simulated $\hatV$ on $\Psi$.} 
Next, we can similarly write the state of the simulated $\hatV$ at the end of round $i$, denoted by $\Psi_i$, as
\[
\Psi_i \coloneqq \expect_{\btau} \sum_{\tau_{\le i}} p_{\sigma^{\btau},a,b,r,\tau_{\le i}} \phi_{\sigma^{\btau},a,b,r,\tau_{\le i}} \otimes \COM^r_{a,b} \otimes \proj{\tau_{\le i}} \otimes \Opens_{a,b,r}^{\tau_{\le i}} \otimes \proj{\btau}.
\]

\newcommand{\event}{\mathcal{E}}
\newcommand{\hPsi}{\widehat{\Psi}}

Let $\event_{i}$ be the event that the guessed sequence $\btau$ has the same length-$(i+1)$ prefix as the simulated sequence $\tau$. From the above, we have
\[
\Pr[\event_i] = \expect_{\btau} p_{\sigma^{\btau},a,b,r,\btau_{\le i}}.
\]

Let $\event_{-1}$ be the trivial event that always happens for notational convenience. 
Moreover, conditioning on $\event_i$, the simulated state of $\hatV$ at the end of round $i$ collapses to
\[
\hPsi_i \coloneqq \frac{1}{\Pr[\event_i]} \cdot \expect_{\btau} p_{\sigma^{\btau},a,b,r,\btau_{\le i}} \phi_{\sigma^{\btau},a,b,r,\btau_{\le i}} \otimes \COM^r_{a,b} \otimes \proj{\btau_{\le i}} \otimes \Opens_{a,b,r}^{\btau_{\le i}}.
\]

For convenience set 
\[
\hPsi_{-1} = \Ex_{\btau} \sum_{a,b,r} \tilde{\sigma}^{\btau}_{a,b} \otimes \COM^r_{a,b} \otimes \xi
\]

\paragraph*{Some useful states.} 

For every $\tau \in [m]^{\ell + 1}$ and $i \in \{0,1,\dotsc,\ell\}$, we define the unnormalized state
\[
\Phi^{\tau}_i = \expect_{a,b,r} p_{\sigma,a,b,r,\tau_{\le i}} \phi_{\sigma,a,b,r,\tau_{\le i}} \otimes \COM^r_{a,b} \otimes \proj{\tau_{\le i}} \otimes \Opens_{a,b,r}^{\tau_{\le i}},
\]
and
\[
\Lambda^{\tau}_i = \expect_{a,b,r} p_{\sigma^\tau,a,b,r,\tau_{\le i}} \phi_{\sigma^\tau,a,b,r,\tau_{\le i}} \otimes \COM^r_{a,b} \otimes \proj{\tau_{\le i}} \otimes \Opens_{a,b,r}^{\tau_{\le i}}.
\]

\paragraph*{Indistinguishability.} In the following, for notational simplicity, when we write $\Psi \approx_c \Phi$ for two partial states $\Psi$ and $\Phi$ that occur in the analysis of $\caS$ on inputs of length $n$, we mean that there is a function $S(n) = n^{\omega(1)}$, such that for every $S(n)$-time quantum algorithm $A$ that takes $S(n)$ qubit as advice, it holds that
\begin{equation}\label{eq:ind-Psi-Phi}
\Big| \Pr[A(\Psi) = 1] - \Pr[A(\Phi) = 1] \Big| \le 1/S(n),
\end{equation}
where $\Pr[A(\Psi) = 1] = \|\Psi\|_1 \cdot \Pr[A\left(\frac{\Psi}{\|\Psi\|_1}\right) = 1]$, and equals $0$ if $\|\Psi\|_1 = 0$. We also say that $A$ and $B$ are $\negl(n)$-indistinguishable. We also write $\Psi \approx_s \Phi$ to denote that there is $S(n) = n^{\omega(1)}$ such that any quantum algorithm $A$ without any restrictions satisfies~\eqref{eq:ind-Psi-Phi}.

Similarly, when we write $A \approx B$ for two quantities $A$ and $B$ that occur in the analysis of $\caS$ on inputs of length $n$, we mean that there is $S(n) = n^{\omega(1)}$ such that $|A - B| \le 1/S(n)$. We also say that $A$ and $B$ are $\negl(n)$-close.

The following claim is standard and is implicitly used in the proof of~\cite[Lemma~5.7]{BroadbentG20}. We provide a proof sketch for completeness.

\newcommand{\bn}{\bar{n}}
\newcommand{\ba}{\bar{a}}
\newcommand{\bb}{\bar{b}}
\newcommand{\rep}{\mathsf{rep}}

\begin{claim}\label{claim:ind-basic}
	Let $S \subseteq [p(n)]$. For every $q(n)$-qubit quantum state $\sigma$, it holds that
	\[
	\Ex_{a,b,r} \tilde{\sigma}_{a,b} \otimes \COM^r_{a,b} \otimes \Opens_{a,b,r}^{S} \approx_c \Ex_{a,b,r} \widetilde{(\sigma_{S} \otimes I_{[p(n)] \setminus S})}_{a,b} \otimes \COM^r_{a,b} \otimes \Opens_{a,b,r}^{S},
	\]
	where $\Opens_{a,b,r}^S$ denotes the opening for qubits in $S$.
\end{claim}
\begin{proofsketch}
	The idea is to apply a standard hybrid argument. Let $\bar{S} = [p(n)] \setminus S$ and let $\ba,\bb \in \bits^{n}$, for each $i \in \{0,1,\dotsc,p(n) - |S|\}$, we set $\rep(a,\ba,i)$ to be the string obtained from $a$ by replacing $a_j$ with $\ba_j$ for the first $i$ elements $j$ in $\bar{S}$. 
	
	We define the following intermediate state for each $i \in \{0,1,\dotsc,p(n) - |S|\}$
	\[
	\Delta_i = \Ex_{a,b,\ba,\bb,r} \tilde{\sigma}_{\rep(a,\ba,i),\rep(b,\bb,i)} \otimes \COM^r_{a,b} \otimes \Opens_{a,b,r}^{S},
	\]
	Note that
	\[
	\Delta_{0} = \Ex_{a,b,r} \tilde{\sigma}_{a,b} \otimes \COM^r_{a,b} \otimes \Opens_{a,b,r}^S,
	\]
	and
	\[
	\Delta_{|\bar{S}|} = \Ex_{a,b,r} \widetilde{(\sigma_S \otimes I_{\bar{S}})}_{a,b} \otimes \COM^r_{a,b} \otimes \Opens_{a,b,r}^S.
	\]
	
	From the hiding property of our commitment scheme and the fact that the commitments for qubits in $\bar{S}$ is never revealed, it follows that $\Delta_{i-1} \approx_c \Delta_i$ for every $i \in [|\bar{S}|]$, which completes the proof.
\end{proofsketch}

The following claim is a direct corollary of~\autoref{claim:ind-basic}.

\begin{claim}\label{claim:ind-cond}
	For every $\tau \in [m]^{\ell + 1}$ and $i \in \{0,1,\dotsc,\ell\}$, $\Phi^\tau_i \approx_c \Lambda^\tau_i$.
\end{claim}
\begin{proof}
	
	By \autoref{claim:ind-basic} and the fact that $\sigma_S \approx_s (\sigma^\tau)_S$, it suffices to show that if there is an algorithm $A$ distinguishing $\Phi^{\tau}_i$ and $\Lambda^{\tau}_i$, then there is an algorithm $B$ with similar complexity that distinguishes
	\[
	\rho_1 = \Ex_{a,b,r} \tilde{\sigma}_{a,b} \otimes \COM^r_{a,b} \otimes \Opens_{a,b,r}^{\tau_{\le i}} ~~~~\text{and}~~~~
	\rho_2 = \Ex_{a,b,r} \tilde{\sigma}^\tau_{a,b} \otimes \COM^r_{a,b} \otimes \Opens_{a,b,r}^{\tau_{\le i}}
	\]
	with the same advantage. Indeed, we can define $B$ as follows: given a state $\rho$, it first simulates $\hat{V}_0,\hat{V}_1,\dotsc,\hat{V}_{i}$ together with responses from the honest prover, and aborts immediately whenever their output does not match $\tau_{\le i}$. If it does not abort in the previous stages, then it simulates $A$ on the resulting state. By definition, the unnormalized states corresponding to the event that $B$ does not abort given input $\rho_1$ and $\rho_2$, are $\Phi^{\tau}_i$ and $\Lambda^{\tau}_i$ respectively. This completes the proof.
\end{proof}

\begin{claim}\label{claim:sim-close}
	For every $i \in \{-1,0,\dotsc,\ell\}$, assuming that $\Pr[\event_{i}] \approx \frac{1}{m^{i+1}}$, it holds that $\hPsi_{i} \approx_c \Phi_i$.
\end{claim}
\begin{proof}
	We have
	\begin{align*}
	\hPsi_{i} &= \frac{1}{\Pr[\event_{i}]} \cdot \expect_{\btau} p_{\sigma^{\btau},a,b,r,\btau_{\le i}} \phi_{\sigma^{\btau},a,b,r,\btau_{\le i}} \otimes \COM^r_{a,b} \otimes \proj{\btau_{\le i}} \otimes \Opens_{a,b,r}^{\btau_{\le i}}\\	
	&\approx_c \frac{1}{\Pr[\event_{i}]} \Ex_{\tau} \Lambda_{i}^{\tau} \tag{from the definition of $\Lambda_{i}^\tau$}\\
	&\approx_s m^{i+1} \cdot \Ex_{\tau} \Lambda_{i}^{\tau} \tag{from the assumption that $\Pr[\event_{i}] \approx 1/m^{i+1}$}\\
	&\approx_c m^{i+1} \cdot \Ex_{\tau} \Phi_{i}^{\tau} \tag{from~\autoref{claim:ind-cond}}\\
	&= \Phi_{i}. \tag{from the definition of $\Phi_{i}^\tau$}
	\end{align*}
\end{proof}

\begin{claim}\label{claim:prob-event}
	For every $i \in \{0,1,\dotsc,\ell\}$, $\Pr[\event_{i}] \approx \frac{1}{m^{i+1}}$.
\end{claim}
\begin{proof}
	
	We will show that $\Pr[\event_{i}] \approx 1/m^{i+1}$ for every $i \in \{-1,0,\dotsc,\ell\}$, by an induction over $i$. By the definition of $\event_{-1}$, the base case holds.
	
	Next, for every $i \in \{0,1\dotsc,\ell\}$, assuming that $\Pr[\event_{i-1}] \approx 1/m^i$, we will prove that $\Pr[\event_{i} | \event_{i-1}] \approx 1/m$, which implies $\Pr[\event_{i}] \approx 1/m^{i+1}$.
	
	By~\autoref{claim:sim-close}, we have $\hPsi_{i-1} \approx_c \Phi_{i-1}$. Hence, for every $\tau_i \in [m]$, the probability of $\hatV_{i}$ outputs $\tau_i$ given $\hPsi_{i-1}$ or $\Phi_{i-1}$ are $\negl(n)$-close. Therefore, we have
	\begin{align*}
	\Pr[\event_i|\event_{i-1}] &= \Ex_{\btau_i} [\hatV_{i} \text{ outputs $\btau_i$ given $\hPsi_{i-1}$}] \tag{by the definition of $\event_i$}\\
	&\approx \Ex_{\btau_i} [\hatV_{i} \text{ outputs $\btau_i$ given $\Phi_{i-1}$}] \tag{$\hPsi_{i-1} \approx_c \Phi_{i-1}$}\\
	&=1/m,
	\end{align*}
	the last equality holds since the state $\Phi_{i-1}$ does not depend on $\btau_i$.
\end{proof}

Finally, we are ready to prove~\autoref{lemma:zero-knowledge}.
\begin{proof}
	From~\autoref{claim:prob-event}, we know that $\caS$ does not abort with probability $\Pr[\event_{\ell}]$, which is $\negl(n)$-close to $1/m^{(\ell + 1)}$. Note that $m^{(\ell + 1)}$ is polynomial in $n$ since $m$ is polynomial in $n$ and $\ell = O(1)$.
	
	Next, conditioning on the event that $\caS$ does not abort (\ie, $\event_\ell$), $\caS$ outputs a state $\hPsi_{\ell}$ such that $\hPsi_{\ell} \approx_c \Phi_\ell$ by~\autoref{claim:sim-close}.
	
	Hence, we can keep running $\caS$ until it does not abort. This gives us a simulator with $\poly(n)$ expected running time, whose output state is $\negl(n)$-indistinguishable to the actual output state $\Phi_{\ell}$ of $\hatV$ when interacting with the honest prover.
\end{proof}

\subsection{Consequence of $\QPCP$ and Other Instantiations of $\Pizk$}\label{sec:generalizations}

In this subsection, we discuss some generalizations of our results and the implications of our results if $\QPCP$ holds.

\paragraph*{Zero-knowledge proofs from post-quantum OWFs.} Similar to~\cite[Section~1.5]{BroadbentG20}, we can replace the non-interactive commitment schemes in~\autoref{lemma:c-and-s} and~\autoref{lemma:zero-knowledge} by a two-message computationally hiding and statistically binding commitment scheme, at the cost of increasing the round complexity by one (since now the verifier has to run $\pp \getsR \Setup(1^\lambda)$ and sends $\pp$ to the prover at the beginning, see also~\autoref{remark:rec-run-setup}). 

It is straightforward to verify the proofs of~\autoref{lemma:c-and-s} and~\autoref{lemma:zero-knowledge} go through with minor changes, and we have the following theorem.

\begin{reminder}{\autoref{theo:zk-from-OWFs}}
	Assuming the existence of post-quantum OWFs, there is a constant-round computational zero-knowledge proof system with soundness $s(n) - \negl(n)$\footnote{There is a small loss in the soundness since from post-quantum OWFs, our commitment schemes are only statistically binding instead of perfectly binding.} and completeness $c(n)$ for every $L \in (O(\log n),O(1))$-$\SimQMA_{s(n),c(n)}$.
\end{reminder}

\paragraph*{Statistical zero-knowledge arguments.} Again, similar to~\cite[Section~5.3]{BroadbentG20}, our protocol $\Pizk$ is a statistical zero-knowledge argument if the underlying commitment scheme is statistical hiding and computationally binding. We refer readers to \cite{BroadbentG20} for more discussions on such argument systems since it is not the focus of this work.

\paragraph*{Consequence of $\QPCP_\negl$.} Finally, from \autoref{cor:QPCP-negl-and-LocalQMA},~\autoref{theo:zk-from-OWFs}, and~\autoref{theo:LocalQMA-in-SimQMA}, if $\QPCP_\negl$ holds, then the protocol in~\autoref{theo:zk-from-OWFs} applies to all of $\QMA$.

\begin{corollary}
	Assuming the existence of post-quantum OWFs and $\QPCP_{\negl}$ holds, there are a constant $s \in (0,1)$ and a function $c \colon \N \to [0,1]$ satisfying that $1-c$ is negligible, such that there is a constant-round computational zero-knowledge proof system with soundness $s$ and completeness $c$ for every $L \in \QMA$.
\end{corollary}
